Multi-Robot Decentralized Collaborative SLAM in Planetary Analogue Environments: Dataset, Challenges, and Lessons Learned

Decentralized collaborative simultaneous localization and mapping (C-SLAM) is essential to enable multirobot missions in unknown environments without relying on preexisting localization and communication infrastructure. This technology is anticipated to play a key role in the exploration of the Moon, Mars, and other planets. In this article, we share insights and lessons learned from C-SLAM experiments involving three robots operating on a Mars analogue terrain and communicating over an ad hoc network. We examine the impact of limited and intermittent communication on C-SLAM performance, as well as the unique localization challenges posed by planetary-like environments. Additionally, we introduce a novel dataset collected during our experiments, which includes real-time peer-to-peer inter-robot throughput and latency measurements. This dataset aims to support future research on communication-constrained, decentralized multirobot operations.

==> experimentation_figures.tex <==
%!TEX root = ../main.tex

%<*swarm-slam-solution>
\begin{figure}
    \includegraphics[width=\columnwidth]{viz_graph.pdf}
    \caption{Swarm-SLAM pose graph estimates and GPS ground truth. Absolute Translation Error: 3.74$\pm$1.63 meters.}
    \label{fig:pose-graph-viz}
\end{figure}
%</swarm-slam-solution>

%<*swarm-slam-solution-indv>
\begin{figure*}[h]
    \centering
    % First row of images
    \begin{minipage}[t]{0.29\textwidth}
        \centering
        \includegraphics[width=\textwidth]{viz_graph_0.pdf} % Crop top third
        %\vspace{-1.5em}
        \caption*{(a) Robot 1 estimates} % Label
    \end{minipage}
    %\hspace{-1em} % Adjust horizontal space
    \begin{minipage}[t]{0.29\textwidth}
        \centering
        \includegraphics[width=\textwidth]{viz_graph_1.pdf} % Crop top third
        %\vspace{-1.5em}
        \caption*{(b) Robot 2 estimates} % Label
    \end{minipage}
    %\hspace{-1em}
    \begin{minipage}[t]{0.29\textwidth}
        \centering
        \includegraphics[width=\textwidth]{viz_graph_2.pdf} % Crop top third
        %\vspace{-1.5em}
        \caption*{(c) Robot 3 estimates} % Label
    \end{minipage}

    %\vspace{-0.4em} % Adjust vertical space between rows
    \caption{Swarm-SLAM individual robot pose graph estimates and respective GPS ground truth.}
    \label{fig:swarm-slam-solution-indv}
\end{figure*}
%</swarm-slam-solution-indv>

%<*error-distribution>
\begin{figure}
    \includegraphics[width=\columnwidth]{error_distribution.pdf}
    \caption{Absolute Transation Error Distribution. On the y-axis, we report the percentage of poses with absolute translation error below the value on the x-axis.}
    \label{fig:error-distribution}
\end{figure}
%</error-distribution>

%<*latency>
\begin{figure}
    \includegraphics[width=\columnwidth]{latency.pdf}
    \caption{Inter-robot latency measurements between each pair of robots during the field mission. The plot shows latency values in both directions for all robot pairs, along side the inter-robot distance, illustrating the variability in communication delays and the impact of inter-robot distance on latency. Higher latency values highlight the challenges of maintaining real-time communication in decentralized C-SLAM deployments.}
    \label{fig:latency}
\end{figure}
%</latency>

%<*throughput>
\begin{figure}
    \includegraphics[width=\columnwidth]{throughput.pdf}
    \caption{Inter-robot throughput between each pair of robots during the field mission, measured in both directions. The plot shows data transmission rates ranging from approximately 5 to 20 Mbps when the robots are within communication range, underscoring the tight communication constraints in decentralized C-SLAM systems.}
    \label{fig:throughput}
\end{figure}
%</throughput>

%<*lin-acc>
\begin{figure}
    \includegraphics[width=\columnwidth]{lin_acc.pdf}
    \caption{Linear acceleration magnitude from the onboard LiDAR IMUs. We removed the IMU bias and show the average as a dotted line for better comparison. We can see that the Robot 1 (on wheels) was less affected by vibrations than Robot 2 and 3 (on tracks).}
    \label{fig:lin-acc}
\end{figure}
%</lin-acc>

%<*comm-comp>
\begin{figure}
    \includegraphics[width=\columnwidth]{communication_comparison.pdf}
    \caption{Comparison of communication usage versus total available throughput over time during the field mission. The plot shows the cumulative communication bandwidth utilized by the C-SLAM system against the measured total throughput, highlighting how communication demands increase and eventually exceed available capacity.}
    \label{fig:comm-comp}
\end{figure}
%</comm-comp>

%<*comm-budget>
\begin{figure}
    \includegraphics[width=\columnwidth]{communication_vs_budget.pdf}
    \caption{Communication budget versus total available throughput during the field mission. The plot illustrates the relationship between the communication budget---defined as the number of prioritized inter-robot loop closures---and the cumulative available throughput.}
    \label{fig:comm-budget}
\end{figure}
%</comm-budget>

%<*sim-vs-loops>
\begin{figure}
    \includegraphics[width=\columnwidth]{similarities_vs_loops.pdf}
    \caption{Number of loop closures versus place recognition similarity threshold. The plot categorizes loop closures into correct, incorrect, and failed registrations, showing how varying the similarity threshold impacts the quantity and quality of loop closures. This highlights the trade-offs involved in setting similarity thresholds for optimal performance.}
    \label{fig:sim-vs-loops}
\end{figure}
%</sim-vs-loops>

%<*inliers-vs-loops>
\begin{figure}
    \includegraphics[width=\columnwidth]{nb_inliers_vs_loops.pdf}
    \caption{Number of loop closures versus the number of inlier points during 3D registration. The plot distinguishes between correct and incorrect loop closures, demonstrating how varying the inlier threshold affects the accuracy and quantity of loop closures.}
    \label{fig:inliers-vs-loops}
\end{figure}
%</inliers-vs-loops>

%<*ambiguity>
\begin{figure*}[h]
    \centering
    \begin{minipage}[c]{0.3\textwidth}
        \includegraphics[width=\textwidth]{view_1_81_cropped.png}
    \end{minipage}
    \hspace{-1em} % to reduce spacing between images and symbols
    \begin{minipage}[c]{0.05\textwidth}
        \centering
        +
    \end{minipage}
    \hspace{-1em}
    \begin{minipage}[c]{0.3\textwidth}
        \includegraphics[width=\textwidth]{view_2_151_cropped.png}
    \end{minipage}
    \hspace{-1em}
    \begin{minipage}[c]{0.05\textwidth}
        \centering
        =
    \end{minipage}
    \hspace{-1em}
    \begin{minipage}[c]{0.3\textwidth}
        \includegraphics[width=\textwidth]{view_combined_cropped.png}
    \end{minipage}
    \caption{Ambiguity in LiDAR scan matching, showing two scans with a ScanContext similarity of 0.757 and 381 inlier points during 3D registration. Despite the high similarity and significant number of inliers, the ground truth distance between the two scans is 17.28 meters, illustrating the challenge of accurately distinguishing distinct locations in feature-sparse, flat terrain environments. This example highlights the limitations of current place recognition metrics in differentiating between similar but distinct places.}
    \label{fig:matchingambiguity}
\end{figure*}
%</ambiguity>

==> explanation_figures.tex <==
%!TEX root = ../main.tex
%<*overview>
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{swarm-slam-system-overview.pdf}
    \caption{Swarm-SLAM Overview. Our collaborative SLAM system is fully decentralized and supports intermittent inter-robot communication. Swarm-SLAM takes odometry and raw sensor data as input, performs place recognition and registration to produce loop closures, and dynamically elects a robot among the network neighbors to optimize the multi-robot pose graph.}
    \label{fig:swarm-slam-overview}
\end{figure}
%</overview>

%<*csa-field>
\begin{figure}
    \includegraphics[width=\columnwidth]{csa_field.pdf}
    \caption{Multi-robot experiments at the Canadian Space Agency Mars Yard. In our experiments, three robots simultaneously explored the simulated Martian terrain. The robots collaborated through peer-to-peer communication to map the environment and localize themselves within the landscape, demonstrating the effectiveness of our C-SLAM system in a challenging, planetary analogue setting.}
    \label{fig:csa-field}
\end{figure}
%</csa-field>

%<*field-examples>
\begin{figure*}[h]
    \centering
    % First row of images
    \begin{minipage}[t]{0.175\textwidth}
        \centering
        \includegraphics[width=\textwidth, trim=60 0 0 130, clip]{rocks1.png} % Crop top third
        \vspace{-1.5em}
        \caption*{(a)} % Label
    \end{minipage}
    \hspace{-1em} % Adjust horizontal space
    \begin{minipage}[t]{0.175\textwidth}
        \centering
        \includegraphics[width=\textwidth, trim=60 0 0 130, clip]{rocks2.png} % Crop top third
        \vspace{-1.5em}
        \caption*{(b)} % Label
    \end{minipage}
    \hspace{-1em}
    \begin{minipage}[t]{0.175\textwidth}
        \centering
        \includegraphics[width=\textwidth, trim=60 0 0 130, clip]{rocks3.png} % Crop top third
        \vspace{-1.5em}
        \caption*{(c)} % Label
    \end{minipage}

    %\vspace{-0.4em} % Adjust vertical space between rows

    % Second row of images
    \begin{minipage}[t]{0.175\textwidth}
        \centering
        \includegraphics[width=\textwidth, trim=60 0 0 130, clip]{ambiguity0.png} % Crop top third
        \vspace{-1.5em}
        \caption*{(d)} % Label
    \end{minipage}
    \hspace{-1em}
    \begin{minipage}[t]{0.175\textwidth}
        \centering
        \includegraphics[width=\textwidth, trim=60 0 0 130, clip]{ambiguity1.png} % Crop top third
        \vspace{-1.5em}
        \caption*{(e)} % Label
    \end{minipage}
    \hspace{-1em}
    \begin{minipage}[t]{0.175\textwidth}
        \centering
        \includegraphics[width=\textwidth, trim=60 0 0 130, clip]{dynamic0.png} % Crop top third
        \vspace{-1.5em}
        \caption*{(f)} % Label
    \end{minipage}
    \vspace{-0.4em} % Adjust vertical space between rows
    \caption{Images of the Canadian Space Agency Mars Yard terrain captured by cameras onboard the robots. Images (a) to (e) illustrate the diverse and challenging features of the terrain. Panel (f) demonstrates instances where the robots are occasionally within line-of-sight of each other, acting as challenging dynamic objects.}
    \label{fig:terrain-pictures}
\end{figure*}
%</field-examples>

%<*robot>
\begin{figure}
    \includegraphics[width=\columnwidth]{robots.pdf}
    \caption{Robot design: The base of the robots are an AgileX Scout 2.0 Rover (Robot 1) and AgileX Bunkers (Robot 2 and 3). Each robot is equipped with a LiDAR, IMU sensor suite, and an ad-hoc networking router enabling peer-to-peer communication.}
    \label{fig:robots}
\end{figure}
% \begin{figure}
%     \includegraphics[width=\columnwidth]{Bunker.pdf}
%     \caption{Robot 2 and 3 design: The robots are based on AgileX Bunker platforms, featuring the same sensor suite as Robot 1. These robots are equipped with tracks, enhancing mobility over rough terrain.}
%     \label{fig:robot1}
% \end{figure}
%</robot>

%<*gps>
\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{basestation_gps.jpg}
    \caption{GPS RTK Station.}
    \label{fig:gps}
\end{figure} 
%</gps>

%<*datasettable>
\begin{table}[t]
    \vspace{4mm}
    \centering
    \caption{Content per robot of our novel dataset~\cite{lajoieCollaborativeSimultaneousLocalization2024}, comprising SLAM and inter-robot communication sensing data.}
    \ra{1.0}
    \begin{tabular}{@{}lcrr@{}}\toprule
        Sensor & Data Types & Frequency (Hz) \\\bottomrule
        \multirow{2}{*}{\centering Ouster LiDAR OS0} & Point Clouds & 9.81 \\
        & IMU & 98.54 \\
        & TF frames & 624.78 \\\hline
        VectorNav VN-100 & IMU & 196.32 \\\hline
        \multirow{4}{*}{\centering GL iNet AX1800} & \vspace{-0.5em}Pairwise latency with  & \multirow{2}{*}{\centering 0.92} \\
        & each other robot (ms) & \\
        & \vspace{-0.5em}Pairwise throughput with & \multirow{2}{*}{\centering 0.93} \\
        & each other robot (Kbps) & \\\hline
        U-Blox ZED F9 GPS & GPS fix & $\sim1.0$ \\\bottomrule
    \end{tabular}
    \label{tab:dataset_table}
\end{table}
%</datasettable>
